A real-time full-chain wearable sensor-based musculoskeletal simulation: an OpenSim-ROS Integration

Musculoskeletal modeling and simulations enable the accurate description and analysis of the movement of biological systems with applications such as rehabilitation assessment, prosthesis, and exoskeleton design. However, the widespread usage of these techniques is limited by costly sensors, laboratory-based setups, computationally demanding processes, and the use of diverse software tools that often lack seamless integration. In this work, we address these limitations by proposing an integrated, real-time framework for musculoskeletal modeling and simulations that leverages OpenSimRT, the robotics operating system (ROS), and wearable sensors. As a proof-of-concept, we demonstrate that this framework can reasonably well describe inverse kinematics of both lower and upper body using either inertial measurement units or fiducial markers. Additionally, we show that it can effectively estimate inverse dynamics of the ankle joint and muscle activations of major lower limb muscles during daily activities, including walking, squatting and sit to stand, stand to sit when combined with pressure insoles. We believe this work lays the groundwork for further studies with more complex real-time and wearable sensor-based human movement analysis systems and holds potential to advance technologies in rehabilitation, robotics and exoskeleton designs.

==> input/03_3_pipeline_rmse_old.tex <==

\newcommand{\MyTableNum}[2]{#1}
%\newcommand{\MyTableNum}[2]{\qty{#1}{#2}}



\begin{table}
 \caption{RMSE\parnote{Root mean square error computed from difference between platform full real-time pipeline output and Vicon offline manually processed output\frederico{move the units to the angle and torque and make the angle and torque vertical multi line}} for IK and ID for different movements investigated.\frederico{write individual values, s1 s2}}
    \label{tab:full_rmse}
\begin{minipage}{\columnwidth}
\begin{tabularx}{\textwidth}{G{1cm}C *{3}{S[round-mode = places,table-column-width = 2cm]}  }
\toprule
                          &   & \textbf{Walking} 		                                      & \textbf{Sts}                                                 & \textbf{Squat}               \\
\midrule
\multicolumn{4}{l}{\textbf{Angle}} \\

& Hip Flex/Ext            & \MyTableNum{4.563904984722703   }{\degree}                 & \MyTableNum{7.459864363732104    }{\degree}                & \MyTableNum{7.146453342231593  }{\degree}\\ 
& Knee Flex/Ext                 & \MyTableNum{3.884305741238474   }{\degree}                 & \MyTableNum{5.491276591132661    }{\degree}                & \MyTableNum{11.237005926397725 }{\degree}\\ 
& Ankle Dors/Plan                 & \MyTableNum{5.119722281869612   }{\degree}                 & \MyTableNum{3.3232547509208543   }{\degree}                & \MyTableNum{7.255564019053076  }{\degree}\\ 
\multicolumn{4}{l}{\textbf{Torque}} \\

& Hip Flex/Ext           & \MyTableNum{0.793403919201053   }{\newton\meter\per\kilogram}  & \MyTableNum{0.13673672913688859  }{\newton\meter\per\kilogram} & \MyTableNum{0.10785129983997689}{\newton\meter\per\kilogram}\\ 
& Knee Flex/Ext                  & \MyTableNum{0.5171355142319838  }{\newton\meter\per\kilogram}  & \MyTableNum{0.12195277321802445  }{\newton\meter\per\kilogram} & \MyTableNum{0.2503595332168255 }{\newton\meter\per\kilogram}\\ 
& Ankle Dors/Plan                 & \MyTableNum{0.1831369084072002  }{\newton\meter\per\kilogram}  & \MyTableNum{0.033440887002639294 }{\newton\meter\per\kilogram} & \MyTableNum{0.10117512674277725}{\newton\meter\per\kilogram}\\
%\multicolumn{4}{c}{Activation} \\

%tib ant           & \MyTableNum{0.22313747045510038 }{}                        & \MyTableNum{0.24025856183678418  }{}                       & \MyTableNum{0.1484393863331543 }{}\\ 
%med gas           & \MyTableNum{0.1681924476516033  }{}                        & \MyTableNum{0.30900903944819696  }{}                       & \MyTableNum{0.2063247129712555 }{}\\ 
%soleus            & \MyTableNum{0.17030506543060842 }{}                        & \MyTableNum{0.4332599317846246   }{}                       & \MyTableNum{0.25029588052131196}{}\\ 
%glut max1         & \MyTableNum{0.25297010584585916 }{}                        & \MyTableNum{0.3409461715806866   }{}                       & \MyTableNum{0.26244394703302326}{}\\ 
%vas med           & \MyTableNum{0.34260296875467877 }{}                        & \MyTableNum{0.21969976164550017  }{}                       & \MyTableNum{0.29522808445513166}{}\\ 
\bottomrule
\end{tabularx}
\parnotes
\end{minipage}
\end{table}
